AdaServe: Accelerating Multi-SLO LLM Serving with SLO-Customized Speculative Decoding

Modern large language model (LLM) applications exhibit diverse service-level objectives (SLOs), from low-latency requirements in interactive coding assistants to more relaxed constraints in data wrangling tasks. Existing LLM serving systems, which rely on uniform batching and scheduling strategies, often fail to meet these heterogeneous SLOs concurrently. We present AdaServe, the first LLM serving system designed to support efficient multi-SLO serving through SLO-customized speculative decoding. AdaServe formulates multi-SLO serving as a constrained optimization problem and introduces a hardware-aware algorithm that constructs a speculation tree tailored to each request's latency target. It features a speculate-select-verify pipeline that enables fine-grained control over decoding speed while maximizing system throughput. AdaServe further adapts to workload variation by dynamically adjusting speculation parameters. Evaluations across diverse workloads show that AdaServe reduces SLO violations by up to 4.3$\times$ and improves goodput by up to 1.9$\times$ compared to the best performing baselines, highlighting its effectiveness in multi-SLO serving.

==> abstract.tex <==
\begin{abstract}

Alternative titles: SLO-Aware LLM Serving with Speculative Decoding

% This paper introduces \sys, a system that accelerates generative large language model (LLM) serving with {\em theoretically-optimal} speculative scheduling.

\end{abstract}


==> intro-old.tex <==
\section{Introduction}
\label{sec:intro}

Large language models (LLMs) have significantly advanced the capabilities of various natural language processing tasks, including chatbots, machine translation, virtual assistants, and code generation.
These applications inherently involve diverse Service Level Objectives (SLOs).
For example, in the context of chatbots, LLMs are employed to generate responses at a rate faster than human reading speeds (i.e., 10 tokens per second)~\cite{brysbaert2019many,liu2024andes,zhong2024distserve}.
Integrating LLMs into web search services requires a significantly tighter decoding latency, as users are more likely to abandon the search if the results take too long~\cite{arapakis2014impact,brutlag2008user}.
In more complex application scenarios relying on LLM APIs, inference requests may need to be completed as soon as possible to avoid blocking the execution of other dependent system modules~\cite{298764,khattab2024dspy}.

To improve the overall throughput of LLM serving, existing systems use {\em continuous batching}, which adds new requests and removes completed requests in the current batch at the beginning of each serving iteration~\cite{yu2022orca}.
%
This iteration-level batching approach improves LLM serving throughput and GPU utilization.
%
However, it cannot support requests with customized SLOs since the decoding computation of all requests are batched together in each iteration, achieving {\em identical} time-per-output-token (TPOT) for all requests.
%
As a result, existing LLM serving systems either do not offer SLO guarantees by employing a best-effort approach to serving requests (e.g., OpenAI's APIs~\cite{openai2023gpt4}) or assume a {\em uniform} SLO constraint across all requests assigned to each serving pipeline.
% \ZL{Do we need to say why we don't want to use separate pipelines here? 1. The number of applications are growing. 2. Due to the throughput-latency tradeoff, the fast and slow requests are complementary.}

This paper introduces \Sys, a system for {\em SLO-customized} LLM serving.
%
The key idea behind \Sys is to leverage {\em fine-grained speculative decoding} techniques to enable customized SLOs for individual requests while supporting continuous batching to maintain high throughput.
%
To serve a batch of requests with diverse SLOs, \Sys performs speculative decoding~\cite{chen2023accelerating,leviathan2022fast} and uses a draft model to predict multiple output tokens for each request. Based on the SLO of individual requests, it dynamically selects a subset of speculated tokens for verification, which enables \Sys to maximally attain the request SLOs while achieving high serving throughput.

%
Although speculative decoding (SD) has been employed in existing systems~\cite{miao2023specinfer,medusa,fubreak} to reduce LLM serving latency, \Sys is the first attempt that leverages SD for SLO-customized serving and must address two key challenges. Next, we discuss these challenges and the techniques \Sys uses to overcome them.

First, existing speculative decoding methods generally use a draft model to predict multiple output tokens and verify their correctness in parallel using the LLM. This approach improves the TPOT for individual requests, while also reducing the overall serving throughput due to the cost of speculation and verifying incorrectly speculated tokens.
%
To address this challenge, \Sys uses the logits of the draft model to approximate the probability that each speculated token can be verified by the LLM.
Using these probabilities as input, \Sys introduces a {\em theoretically optimal} algorithm to construct token trees by maximizing the expected number of tokens verified by the LLM.
%
To make this algorithm work in practice and minimize the run-time overhead of speculation, \Sys employs a practical adaptation of the algorithm to account for real-world constraints and uncertainties.
%To minimize the run-time overhead of token tree construction, \Sys employs a practical adaptation of the algorithm to account for real-world constraints and uncertainties.

%
%This approach allows \Sys to opportunistically 

The second challenge \Sys must address is SLO customization. Existing speculative decoding methods generally employ a {\em static} approach to optimize speculative performance and apply a {\em uniform} strategy across all batched requests. This coarse-grained approach does not promote SLO customization at the request level.
%
To address this issue, \Sys introduces a {\em fine-grained speculative decoding} pipeline consisting of four stages, including speculation, SLO-customized selection, throughput-optimized selection, and verification. First, during the \textit{speculation} stage, \Sys constructs a candidate token tree for each request in the batch, containing tokens with high probabilities to be verified by the LLM.
Second, in \textit{SLO-customized token selection}, \Sys calculates the minimum number of tokens each request must accept to fulfill its TPOT SLO and selects enough tokens from the candidate token tree to achieve this goal.
Next, in \textit{throughput-optimized token selection}, \Sys selects additional tokens to fully utilize the remaining budget, thereby enhancing throughput. Together, these two selection steps dynamically construct the token trees in a fine-grained manner to attain customized SLOs while achieving high throughput. Finally, the draft token trees are sent to the LLM for verification.

\paragraph{Evaluation.} We conduct evaluations to compare \Sys with state-of-the-art LLM serving systems and various serving strategies for serving requests from diverse services and applications. The results demonstrate that \Sys consistently outperforms all baselines. In end-to-end comparisons, \Sys achieves up to 73\% higher SLO attainment and 74\% higher goodput than the best baseline systems. Additionally, our evaluations show that \Sys can maintain a 95\% SLO attainment when serving requests with TPOT SLO requirements that are 20\% stricter than the \textit{baseline latency} which represents the profiled lower limit for serving with continuous batching alone.

\ZL{TODO: We can remove the following paragraph and add a paragraph to talk about the contributions instead.}
The rest of the paper is organized as follows: Section \ref{sec:background} provides the background on speculative decoding and key SLO-aware inference serving concepts. \Cref{sec:problem} formulates the SLO-customized serving problem. \Cref{sec:method} details the core speculative scheduling algorithms. \Cref{sec:system} describes the system design and implementation. \Cref{sec:eval} presents our evaluation results. \Cref{sec:related} discusses the related works.

\if 0
\section*{Old Intro}

Large language models (LLMs) have revolutionized many daily tasks thanks to unprecedented capabilities in text generation, translation, and understanding. While these models have exploded in popularity, their deployment in production faces significant challenges, particularly in guaranteeing strict Service Level Objectives (SLOs) while maintaining high throughput and efficiency.

Existing systems 

Speculative decoding~\cite{miao2023specinfer, xiaspeculative, leviathan2022fast, chen2023accelerating} has emerged as a promising technique to accelerate LLM inference by leveraging smaller, faster models to predict the output of larger models. While this approach has shown considerable speedup in single-request scenarios, its application in high-throughput, multi-request serving environments remains challenging~\cite{liu2024optimizingspecdecoding}. The primary difficulties lie in efficiently allocating computational resources across multiple requests and constructing optimal token trees that maximize the number of accepted tokens while adhering to individual request SLOs.

\ZL{
The issues with the batching behavior of current system.
\begin{enumerate}
    \item Not flexible: The latency is bounded by the longest request. Sacrifice the requests with more stringent SLO.
    \item Latency-throughput tradeoff, tight SLO is not achievable or achievable with a very small batch size, limiting the throughput.
    \item Prefilling add overhead to decode (vllm, Sarathi-Serve).
    \item Does not fully utilize the hardware compute resource.
\end{enumerate}
}


This paper introduces \Sys, a novel SLO-aware scheduling system for LLM serving with speculative decoding. This paper introduces several key innovations:
\begin{itemize}
    \item A theoretically optimal token tree construction algorithm that maximizes the expected number of accepted tokens across all requests
    \item A practical adaptation of this algorithm that accounts for real-world system constraints and uncertainties
    \item A LLM inference scheduler that prioritizes requests based on their proximity to SLO violations
    \item An efficient implementation of the techniques above in a distributed LLM inference engine, including optimizations such as CUDA-graph-enabled kernels for small model inference and adaptive tree depth and width control
\end{itemize}

\fi 
